Face, Body, Voice: Video Person-Clustering with Multiple Modalities

The objective of this work is person-clustering in videos -- grouping characters according to their identity. Previous methods focus on the narrower task of face-clustering, and for the most part ignore other cues such as the person's voice, their overall appearance (hair, clothes, posture), and the editing structure of the videos. Similarly, most current datasets evaluate only the task of face-clustering, rather than person-clustering. This limits their applicability to downstream applications such as story understanding which require person-level, rather than only face-level, reasoning. In this paper we make contributions to address both these deficiencies: first, we introduce a Multi-Modal High-Precision Clustering algorithm for person-clustering in videos using cues from several modalities (face, body, and voice). Second, we introduce a Video Person-Clustering dataset, for evaluating multi-modal person-clustering. It contains body-tracks for each annotated character, face-tracks when visible, and voice-tracks when speaking, with their associated features. The dataset is by far the largest of its kind, and covers films and TV-shows representing a wide range of demographics. Finally, we show the effectiveness of using multiple modalities for person-clustering, explore the use of this new broad task for story understanding through character co-occurrences, and achieve a new state of the art on all available datasets for face and person-clustering.

==> sections/protocol.tex <==

Here, we give implementation details and describe the different metrics and test protocols we use.

\noindent
\textbf{Implementation details.}
We use the face, body and voice track annotations and features from \dnameemphasis 
(Sections~\ref{sub:dataset_content},\ref{sub:feature_extraction}). 
For all modalities, we compute the feature distances $d_f$,$d_b$,$d_v$ using (1 - cosine similarity). All features are unit length.  
%
We use the first five episodes of Friends to set the hyper-parameters of \mnameMM to: 
$\tau_f^{\text{tight}}{=}{0.5}$,  $\tau_f^{\text{loose}}{=}0.55$, $\tau_v^{\text{tight}}{=}0.4$,  $\tau_b^{\text{tight}}{=}0.35$, $\rho{=}0.9$ and $\tau_b^{\text{back}}{=}0.4$. 
\todo{More exps solidifying this}. These five episodes are not included in the test set for all experiments and baselines (but the other 20 episodes of Friends are; similarly, baseline results are computed on these 20 episodes). 
Note, these hyper-parameters are fixed for all experiments, and only have to be re-learnt  if the embedding features are changed.
% To test generalisation, we do not tune these parameters on other datasets in \dnameemphasis. 
% \new{To use different input features to those provided with \dnameemphasis, different values for the above hyper-parameters must be learnt. }

%%%%%%%%%%%%%%%
\noindent \textbf{Metrics. }
%\label{sub:metrics}
%%%%%%%%%%%%%%%%%%
For each dataset in \dnameemphasis, we measure each metric at the episode level and then report the average over all episodes. 
Following~\cite{Kalogeiton20,ball}, we use Weighted Cluster Purity (\textbf{WCP}) and Normalized Mutual Information (\textbf{NMI}). 
\noindent WCP weights the purity of a cluster by the number of samples belonging in it. 
NMI~\cite{manning2008introduction}  measures the trade-off between clustering quality and number of resulting clusters.
%
\noindent \textbf{Character Precision and Recall (CP, CR) }are computed using the number of ground truth clusters/identities. Each identity is uniquely assigned to a cluster. CP is the proportion of tracks in a cluster that belong to its assigned character, while CR is the proportion of that character's total tracks that appear in the cluster. These are averaged across all characters, thus weighting each equally.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Test Protocol}
\noindent
\textbf{Test protocol.}
We \new{evaluate: }i.\ automatic termination (AT), \ie unknown number of clusters, and ii.\ oracle cluster (OC), when known. 
AT is realistic for applications, while OC offers a fair comparison to the state of the art.

\begin{comment}
\noindent 
\textbf{Person-Clustering.}
Here, we conduct experiments on all person-track annotations. 
\textbf{Baselines.} 
We are the first to evaluate this on \dnameemphasis, so we compare to two strong baselines, based on the best existing face-clustering algorithm, C1C~\cite{Kalogeiton20}. (i) The first baseline uses C1C to cluster body rather than face features. This ignores the person-tracks without bodies (< 2\% of person tracks) and is inspired by person re-id, that uses body features alone. (ii) For the second, we use regular C1C to cluster faces, with the addition of Stage 3 of \mnameMM for clustering face-less bodies.

\noindent 
\textbf{Face-Clustering.} 
In order to compare to previous work, we provide experimental results on the more limited task of face-clustering, by evaluating only the face-tracks. In this setting we do not have access to the person-tracks without faces, although we do have access to the additional modalities of existing face-tracks, \ie the associated body-track and voice (if exists). We provide experiments both with only using only face-tracks, and with using all modalities. In line with previous work~\cite{Kalogeiton20}, performance is evaluated at the detection level. 
%
\textbf{Baselines.} 
We compare to C1C~\cite{Kalogeiton20}, Ball Cluster Learning~\cite{ball} and FINCH~\cite{finch}. \todo{Reviewer asked which Finch partition}
For TBBT and Buffy, we evaluate using the same face-tracks and annotations as in ~\cite{Kalogeiton20,ball}. 
For Friends and Sherlock, we use official re-implementations of FINCH and C1C.  These present different numbers to those reported in~\cite{Kalogeiton20}, where either backs of heads are clustered (Friends), or several incorrect annotations are used (C1C).  
\vic{note sure: maybe move the following to experiments?}
Note, we do not compare to~\cite{sharma2019self_before34,sharma2019video34,rothlingshofer2019self} that use older, \new{and less challenging} annotations for TBBT and Buffy.
Since \mnameMM outperforms all state of the art, we argue that it would also outperform these older methods.
\end{comment}









==> sup/Supplementary_Video_Contents.tex <==

Three videos are included with this supplementary material. Here, we explain what is contained in each of them. 

The first is titled, ``Story\_Understanding''. This video highlights the advantages of the new task of multi-modal video person-clustering, over the established, more limited task of face-clustering. The video visualises the amount of information that is used by these two tasks. For the face-clustering task, only information from visible faces is used. This omits important information such as characters viewed from behind, or from the audio track. This limits the utility of the resulting clusters for downstream applications such as story understanding. The multi-modal person-clustering task on the other hand uses all available cues (\ie face, body and voice). Clearly, a person-level understanding is essential for downstream applications of grouping-by-identity such as story understanding.

The second is titled ``VPCD\_Contents''. This video visualises the different annotations provided in \dnameemphasis, namely the face-tracks, body-tracks (from front and behind), and voice-tracks. The video shows clips containing example annotations from all 6 program sets in \dnameemphasis. Every face-body pair belonging to the same person-track is drawn with the same color. Note,  \dnameemphasis covers a diverse set of characters in a variety of scenes (\eg including dark scenes in Sherlock, Hidden Figures), various viewpoints and over-the-shoulder shots. 

The third video, titled ``MuHPC\_Results'' shows a selection of \mnameMM person-clustering results from \dnameemphasis. In each clip, tracks are marked with a unique cluster ID number and colour, which signify which cluster they belong to. Particularly of note are the multiple backs of people that are clustered correctly \ie Ross (cluster 2) in the first clip from Friends, Penny (cluster 3) in the second clip from TBBT, and the multiple backs in the dark scene from Buffy. Impressively, the very small Chandler, Joey and Ross tracks (clusters 1,0,2, respectively) at the back of the shot at the end of the Friends clip, are correctly clustered with other tracks of the same character.


==> sup/qual_results.tex <==
Further qualitative examples of the clustering process for characters in two of the program sets in \dnameemphasis are shown in Figure~\ref{fig:qual_clust}. In both cases, Stage 1 is shown to produce high-precision clusters of the character. The face alone cannot confidently merge these clusters, due to
each cluster containing different views of the same character (\eg frontal and profile). These clusters are merged via speaking person-tracks, using the multi-modal bridges of Stage 2. Back views of the same character are then merged into the clusters in Stage 3. The resulting clusters contain differing views of the same character, with varying pose, lighting conditions, and camera viewpoints, all while maintaining high precision.

\input{figures/qual_fig}

==> tables/AT_person_cluster.tex <==
\begin{table*}[ht!]
\centering
\resizebox{\linewidth}{!}{
\footnotesize{
\begin{tabular}{llccc|ccccccccccccccccccccccc}
\toprule
\# & Method & \multicolumn{3}{c|}{Modalities}   & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{TBBT}}  }       &\cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}}  &                                                             & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Buffy}} }        &          \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 165}}                  &                                & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Sherlock}}}  &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 50}}  &  & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Friends}}} & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 239}}\\ 
%%%%%%%%%%%%%%%%%%%%
& \multicolumn{1}{l}{} & face & body & voice  & WCP                  & NMI                  & CP            & CR      & \multicolumn{1}{c}{$\#C_p$} & & 
WCP                  & NMI                  & CP     & CR            & \multicolumn{1}{c}{$\#C_p$} & & 
WCP                  & NMI                  & CP      & CR            & \multicolumn{1}{c}{$\#C_p$} & &
WCP                  & NMI                  & CP       & CR           & $\#C_p$ \\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% i & \multirow{2}{*}{Baseline} &  & \checkmark & &  66.2             &       54.9               &       11.4           &     & \multicolumn{1}{c}{33.0} &    &        52.0             &       48.8               &       40.6  &              & \multicolumn{1}{c}{24.6}  &  &         60.3             &          24.0            &        10.7  &             & \multicolumn{1}{c}{36.0}   &  &        62.8              &           56.0           &       49.8   &             & 56.4    \\ 
ii & baseline &  \checkmark & \checkmark &  &     81.7          &   77.7                   &    28.7        &  39.5        & \multicolumn{1}{c}{41}    &   &    56.1             &      50.9                               & \multicolumn{1}{c}{12.5} & 24.2   &        40         &                   &        74.7           & \multicolumn{1}{c}{42.1}    &  20.2       &    37.4        &  25             &                     & 83.7  &  80.2  & 58.6 & 69.5 &    185\\ \hline
%%%%%%%%%%%%%%%%%%%%
% iii & \multirow{3}{*}{\mnameMM}  &   \checkmark & \checkmark &   &    \textbf{97.0}              &         92.9             &         \textbf{77.6}             & \multicolumn{1}{c}{79.6}  &   &          \textbf{86.4}            &         76.3             &         69.5             & \multicolumn{1}{c}{69.9}  &   &           80.3           &         47.4             &         46.8             & \multicolumn{1}{c}{49.7}    & &              90.0        &             82.3         &             \textbf{88.4}         & 82.6    \\
%%%%%%%%%%%%%%%%%%%
% iv &  & \checkmark & \checkmark &   &  \checkmark &  &     \textbf{97.0}            &          92.9            &      76.7                & \multicolumn{1}{c}{79.5}  &   &       85.9 &  76.1             &           69.0           &        \multicolumn{1}{c}{69.5}   &  &      79.4                &       50.9               &     58.6                 & \multicolumn{1}{c}{53.3}  &   &     89.5                 &      82.8               &        87.1           &    83.1    \\
 %%%%%%%%%%%%%%%%%%%%%%%%%% second row
% v &  & \checkmark &\checkmark  & \checkmark &  & \checkmark &      96.8               &     \textbf{93.2}                 &     76.9                 & \multicolumn{1}{c}{79.1}    & &           86.0           &      76.6               &       69.8               & \multicolumn{1}{c}{70.6}   &  &     78.5                 &        50.3              &          57.4            & \multicolumn{1}{c}{\textbf{55.1}}    & &   \textbf{90.8}                   &     83.4                 &          87.0            & \textbf{85.4}  \\  \hline 
%%%%%%%%%%%%%%%%
vi & \cellcolor{mistyrose}{\mnameMM} &  \checkmark  & \checkmark & \checkmark &      97.8             & 94.1           &  86.6          &     83.2      & \multicolumn{1}{c}{139}   &  &       87.3               &        77.8             &      82.4   &  80.5          & \multicolumn{1}{c}{197}  &   &      80.8              &       54.0               &   64.9   &    54.4    & \multicolumn{1}{c}{50}  &   &93.9                    &        86.0            &   94.1       &    88.2       &    454  \\
\bottomrule
%%%%%%%%%%%%%%%%%%%%%%%% new one
%%%%%%%%%%%%%%%%%%%%%%%%
\# &Method & \multicolumn{3}{c|}{Modalities}    &  \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Hidden Figures}}}   & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 24}}  & & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{About Last Night}} } &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 10}}    & &  \multicolumn{5}{c}{{\textbf{}}} & &  \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Average}} } & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 618}}                                                                 \\ 
%%%%%%%%%%%%%%%%%%%%
& \multicolumn{1}{l}{} & face & body & voice   & WCP                  & NMI                  & CP       &  CR        & \multicolumn{1}{c}{$\#C_p$}  & & WCP                  & NMI                  & CP       &   CR       & \multicolumn{1}{c}{$\#C_p$} &  &                   &                   &           &       & \multicolumn{1}{c}{} &  &
WCP                  & NMI                  & CP          &  CR     & $\#C_p$                  \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% i &\multirow{2}{*}{Baseline} &  & \checkmark & &                 33.7          &           10.5          &           17.6     &      & \multicolumn{1}{c}{31.7}    & &                27.3      &       17.9               &       19.9        &       & \multicolumn{1}{c}{19.3}   &  &                     &             &       &                  &       \multicolumn{1}{c}{}   &      & 50.4 & 35.4 & 25.0 & & 33.5      \\ 
ii & baseline &  \checkmark & \checkmark &       &      55.2             &      52.4           &        23.3      & 33.0    & \multicolumn{1}{c}{11}    &                     &         75.5         &     51.9          & \multicolumn{1}{c}{29.7} & 46.4  & 6                  &                     &                 & \multicolumn{1}{c}{}    &                     &             &        &                  &  71.2     & 59.2 & 28.8 & 41.7&308  \\ 
\hline
% iii & \multirow{3}{*}{\mnameMM}   &   \checkmark & \checkmark & & &       &            71.9          &         61.8             &         56.9             & \multicolumn{1}{c}{48.4}  &   &    81.6                  &         60.1             &         60.7           &  \multicolumn{1}{c}{70.8}  &   &                      &                      &                 & \multicolumn{1}{c}{}  &   &      84.5 & 70.1 & 66.7 & 66.8                \\
%%%%%%%%%%%%%%%%%%%
% iv & & \checkmark & \checkmark &   &  \checkmark &  &               \textbf{73.4 }               &       \textbf{ 63.8 }             &         \textbf{ 62.7   }         & \multicolumn{1}{c}{\textbf{50.8}}   &  &        82.2              &        61.8              &          70.7            & \multicolumn{1}{c}{78.8}  &   &                      &                      &      &        \multicolumn{1}{c}{}   &      &       84.6 & 71.4 & 70.8 & 69.2               \\
 %%%%%%%%%%%%%%%%%%%%%%%%%% second row
% v & & \checkmark &\checkmark  & \checkmark &  & \checkmark &         71.8            &         62.1            &         55.0             & \multicolumn{1}{c}{47.2}   &  &      \textbf{82.6}               &        62.6              &            \textbf{88.2}          & \multicolumn{1}{c}{\textbf{80.0}}   &  &                      &                      &          &        \multicolumn{1}{c}{}  &   &          84.4 & 71.4 & 72.4 & 69.6            \\ \hline
%%%%%%%%%%%%%%%%
vi & \cellcolor{mistyrose}{\mnameMM} &  \checkmark  & \checkmark & \checkmark &       83.3             &    71.9           &    75.9      & 55.7       & \multicolumn{1}{c}{115}  &   &             83.8         &      63.6              &      89.4      &    78.8     & 36  &   &                      &                      &         &  &        \multicolumn{1}{c}{}   & &          \cellcolor{mistyrose}{\textbf{87.8}} & \cellcolor{mistyrose}{\textbf{74.6}} & \cellcolor{mistyrose}{\textbf{82.2}} &\cellcolor{mistyrose}{\textbf{73.5}}  & \cellcolor{mistyrose}{\textbf{991}}            \\
 \bottomrule
\end{tabular}
}}
\caption{\footnotesize{\textbf{Automatic Termination (AT) Person-Clustering Results on \datasetname.} For the TV-shows, each metric is averaged across episodes. The Average, is averaged across all datasets.  $\#C_s$ is the sum number of ground truth clusters across each episode in the dataset. $\#C_p$ is the number of predicted clusters, summed over each episode of the dataset. We report the strong baseline ii (Section 5 in main manuscript), and out full method \mnameMM. The notation ii and vi is taken from Table 2 in the main manuscript.}}
\label{tab:person_results_AT}
% Results on the proposed \datasetname. Method 1 is not using any of the multi-modal bridges in Stage 2. Method 2 is using the bridges. Baseline 1: We replace the primary modality in Stage 1 with the body modality, using the same MovieNet trained features. Method 3: We replace these features with powerful person Re-ID features. 
\end{table*}


==> tables/ablations.tex <==
% %%%% example 
% \begin{table}[t]
% \begin{minipage}[b]{0.4\linewidth}
% \centering
% \resizebox{\linewidth}{!}{
% \footnotesize{
% \begin{tabular}{l|cccrcc}
% \toprule
%       & \multicolumn{2}{c}{\cellcolor{lavenderblue}{TBBT}} &\cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}} &    & \multicolumn{2}{c}{\cellcolor{lavenderblue}{Friends}}  \\ 
%      $\tau_f^{\text{tight}}$  & WCP & NMI & $\#C_p$ & & WCP & NMI \\ \midrule
% 0.40  &  98.5   &      92.9             & 231    &  &                         \\
% 0.45 &  98.2   &        93.9            &  195  &  &                        \\
% 0.50  &   97.8  &    94.1               & 139    &  &                   \\
% 0.55 &    96.8 &    94.0                & 120   &  &                \\     
% 0.60 &    96.0 &    93.5                & 99   &  &                \\     
% \bottomrule
% \end{tabular}
% }}
% \captionof{table}{\small{\textbf{Parameter sweep for the nearest neighbour distance threshold, $\tau_f^{\text{tight}}$.} } }
% \label{tab:ablation1}
% %\vspace{4mm}
% \end{minipage}
% \hspace{0.25cm}%
% \begin{minipage}[b]{0.56\linewidth}
% \centering
% \resizebox{\linewidth}{!}{
% \footnotesize{
% \begin{tabular}{lc|cccccc}
% \toprule
%                       & modality & b           & v          & b           & v          & b           & v          \\ \midrule
%                       & value    & \multicolumn{2}{c}{0.55} & \multicolumn{2}{c}{0.60} & \multicolumn{2}{c}{0.65} \\ \midrule
% \multirow{3}{*}{face} & 0.4      &             &            &             &            &             &            \\
%                       & 0.45      &             &            &             &            &             &            \\\bottomrule      
% \end{tabular}
% }}
% %\vspace{3mm}
% \captionof{table}{\footnotesize{\textbf{Multi-modal bridging ablation. Recomputing these as they were wrong} %We report \todo{xxxxxx aidfhadifa foakdsfjalfd}
% }}
% \label{tab:ablation2}
% \end{minipage}
% \end{table}

\begin{table}[t]
\centering
\resizebox{0.8\linewidth}{!}{
\footnotesize{
\begin{tabular}{l|cccrccc}
\toprule
      & \multicolumn{2}{c}{\cellcolor{lavenderblue}{TBBT}} &\cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}} &    & \multicolumn{2}{c}{\cellcolor{lavenderblue}{\textbf{$Friends_s$}}} &\cellcolor{lavenderblue}{\textbf{$\#C_s$ = 90}} \\ 
     $\tau_f^{\text{tight}}$  & WCP & NMI & $\#C_p$ & & WCP & NMI& $\#C_p$  \\ \midrule
0.40  &  98.5   &      92.9             & 231    &  & 95.8  & 84.6 & 312                       \\
0.45 &  98.2   &        93.9            &  195  &  &  95.3 & 85.2 & 209                      \\
0.50  &   97.8  &    94.1               & 139    &  &  94.7 &85.7 & 147                 \\
0.55 &    96.8 &    94.0                & 120   &  &  94.3 & 85.7 & 120              \\     
0.60 &    96.0 &    93.5                & 99   &  & 94.2 & 85.7 & 111               \\     
\bottomrule
\end{tabular}
}}
\captionof{table}{\small{\textbf{\todo{Remake this with new data} Parameter sweep for the nearest neighbour distance threshold, $\tau_f^{\text{tight}}$.} Results are shown for TBBT and the first 10 episodes of Friends, termed $Friends_s$, for the AT protocol.  } }
\label{tab:ablation1}
%\vspace{4mm}
\end{table}


==> tables/backs.tex <==
\begin{table}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|rrrrrrrrrrrrrrr}
\toprule
dataset       & \cellcolor{lavenderblue}{TBBT} &  & \cellcolor{lavenderblue}{Buffy} & & \cellcolor{lavenderblue}{Sherlock} & & \cellcolor{lavenderblue}{Friends} & & \cellcolor{lavenderblue}{ALN} &  & \cellcolor{lavenderblue}{HF} & & \cellcolor{lavenderblue}{Hannah} & & \cellcolor{lavenderblue}{AVG} \\ \midrule
Accuracy &   xx  & &  xx   &  &  xx   &   &  xx  & &xx &  & xx & & xx &&   xx   \\
Ignored  &   xx  & &  xx   &  &  xx   &   &  xx  & &xx &  & xx & & xx && xx  \\ \bottomrule
\end{tabular}
}
\caption{\footnotesize{\textbf{Back-body clustering accuracy.} For each dataset in \dnameemphasis, the \% accuracy for clustering backs of bodies in Stage 3, along with the \% proportion of bodies not assigned a label for lack of confidence.}}
\label{tab:back_accuracy}
\end{table}

==> tables/face_clustering2.tex <==
% \begin{table*}[!hpt]


\begin{table*}[]
\centering
{\setlength\tabcolsep{3pt}  % default: 6pt --> to decrease the padding between columns 
\resizebox{\linewidth}{!}{
%\small{
\begin{tabular}{lc|rrrrcr rrrrcr rrrrcr rrrrcr rrrrc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multirow{2}{*}{protocol} & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{TBBT}}}  & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}}  &        & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Buffy}}}  &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 165}}  &       & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Friends}}}   & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 239}}  &    & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Sherlock}}} &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 50}} & & 
 \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Average}}} &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = XX}}  \\
\multicolumn{1}{c}{}                        &                           & WCP   & NMI   & CP    & CR    & $\#C_p$ & & WCP   & NMI   & CP    & CR    & $\#C_p$ & & WCP   & NMI   & CP    & CR    & $\#C_p$ & & WCP  & NMI  & CP   & CR   & $\#C_p$  &   
& WCP   & NMI   & CP    & CR    & $\#C_p$ 
\\ \hline
% Finch                                       & AT                        &  65.39     & 55.06      &     0.213  &    0.287   &     &       &       &       &       &     &       &       &       &       &     &      &      &      &      &     \\
BCL~\cite{ball}                                        & AT                        & 90.8 & 85.7 &   -    &    -   & 83  & & 85.0 & 78.8 &  -     &    -   & 121  & &     -  &   -    &    -   &  -     &   -  & &  -    & -     &  -    &   -   &     \\
C1C~\cite{Kalogeiton20}                                          & AT                        &   89.2    &  87.4     &  29.1     &  40.9     &   41   &      &   66.3    &  68.8     & 14.9      &    27.1  &  40  & & 88.2  &  89.8     &  62.4     &     73.2  & 185 & &  76.3&  50.3    & 20.2     & 41.0     &     25      \\
\mnameMM--                                      & AT                        & \textbf{99.4}  & \textbf{97.8}    & \textbf{87.8} & \textbf{88.6} & 168 && \textbf{96.1}  & 92.8  & 85.6 & \textbf{85.5} & 223& & \textbf{98.7} & 94.9 & 98.1 & 94.0 & 543 & & \textbf{86.7}   & 60.3     &79.1     & 71.2     & 96     \\
\mnameMM                                     & AT                        & \textbf{99.4}  & \textbf{97.8}    & \textbf{87.8} & \textbf{88.6} & 168 & &  \textbf{96.1}  &  \textbf{93.7}  &  \textbf{85.9} & 84.8 & 221 & & 98.4 & \textbf{95.9} & 97.7 & \textbf{95.3} & 522 & &  86.3   & \textbf{66.0}     & \textbf{78.4}     & \textbf{74.5}     &     86\\ \midrule
Finch~\cite{finch}                                       & OC                        & 90.8  &  80.5     &   46.1    &    44.2   & \multirow{5}{*}{}&  & 82.9  &   75.3    &   49.6    &   41.0    & \multirow{5}{*}{} & & 92.2   &  89.9     &     85.2  &    85.6   & \multirow{5}{*}{} & &  81.6 &  58.6    &  \textbf{59.8}    &     56.8 & \multirow{5}{*}{}  \\
BCL~\cite{ball}                                         & OC                        & 94.0    & 85.0    &   -    &      - &  &  & 86.5  & 77.6  &  -     &  -     &  &   &    -   &    -   &   -    &      - &   &  &  -    &    -  &      -&     - &   \\
C1C~\cite{Kalogeiton20}                                         & OC                        & 95.3  & 84.5  &   54.9    &  57.3   &    & & 88.1  & 79.1  &    58.1   &  55.4     &    & & 94.3 & 93.2 & 79.1  & 85.5 &   & &  81.6 & 53.8 &     40.5 & 51.7     &    \\
\mnameMM--                                      & OC                        & \textbf{99.1}  & \textbf{97.4}  & \textbf{79.3}  & \textbf{83.0}  &   & & \textbf{95.6}  &  92.2  & \textbf{72.3}  & \textbf{73.8}  &    & & 96.3 & 92.7 & 89.0  & 88.8  & &    & 84.0 & 56.5 & 55.4 & 59.9 &    \\
\mnameMM                                    & OC           &   \textbf{99.1}    &  \textbf{97.4}     &   \textbf{79.3}    & \textbf{83.0}  &  &   &  \textbf{95.6}       &  \textbf{93.1}       &    71.5   &    73.2   &  &   &  \textbf{97.1}     & \textbf{94.6}      &    \textbf{92.3}   & \textbf{92.6}      &  &   &    \textbf{85.1}  &     \textbf{63.9} & 59.6     &  \textbf{62.9}    &    \\ \bottomrule
% MM-HPC3                                     & OC      &       &       &       &       & "   &       &       &       &       & "   &       &       &       &       & "   &      &      &      &      & "  \\ \bottomrule
\end{tabular}
}%}
}
%\vspace{-2mm}
\caption{\footnotesize{
\textbf{Face Clustering Results.} Comparisons to previous state of the art on four datasets, using only face-tracks. We experiment with unknown (AT), and known (OC) number of clusters. We report metrics averaged over each episode in each dataset, and the number of predicted clusters, summed over each episode of the dataset ($\#C_p$). 
MM-HPC-- uses only face, 
whereas MM-HPC uses the multi-modal bridges for body and voice. Where not reported in respective publications, additional numbers are computed using official implementations. Finch has no stopping criterion so results for AT are not reported.}}
\vspace{-2mm}
\label{tab:face_results}
\end{table*}



==> tables/face_clustering_results.tex <==
% \begin{table*}[!hpt]


\begin{table*}[]
\centering
%{\setlength\tabcolsep{7.5pt}  % default: 6pt --> to decrease the padding between columns 
\resizebox{\linewidth}{!}{
%\small{
\begin{tabular}{lc|rrrrcr rrrrcr rrrrcr rrrrc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multirow{2}{*}{protocol} & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{TBBT}}}  & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}}  &        & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Buffy}}}  &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 165}}  &       & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Friends}}}   & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 239}}  &    & \multicolumn{4}{c}{\cellcolor{lavenderblue}{\textbf{Sherlock}}} &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 50}} \\
\multicolumn{1}{c}{}                        &                           & WCP   & NMI   & CP    & CR    & $\#C_p$ & & WCP   & NMI   & CP    & CR    & $\#C_p$ & & WCP   & NMI   & CP    & CR    & $\#C_p$ & & WCP  & NMI  & CP   & CR   & $\#C_p$  \\ \hline
% Finch                                       & AT                        &  65.39     & 55.06      &     0.213  &    0.287   &     &       &       &       &       &     &       &       &       &       &     &      &      &      &      &     \\
BCL~\cite{ball}                                        & AT                        & 90.8 & 85.7 &   -    &    -   & 83  & & 85.0 & 78.8 &  -     &    -   & 121  & &     -  &   -    &    -   &  -     &   -  & &  -    & -     &  -    &   -   &     \\
C1C~\cite{Kalogeiton20}                                          & AT                        &   89.2    &  87.4     &  29.1     &  40.9     &   41   &      &   66.3    &  68.8     & 14.9      &    27.1  &  40  & & 88.2  &  89.8     &  62.4     &     73.2  & 185 & &  76.3&  50.3    & 20.2     & 41.0     &     25      \\
\mnameMM--                                      & AT                        & \textbf{99.4}  & \textbf{97.8}    & \textbf{87.8} & \textbf{88.6} & 168 && \textbf{96.1}  & 92.8  & 85.6 & \textbf{85.5} & 223& & \textbf{98.7} & 94.9 & 98.1 & 94.0 & 543 & & \textbf{86.7}   & 60.3     &79.1     & 71.2     & 96     \\
\mnameMM                                     & AT                        & \textbf{99.4}  & \textbf{97.8}    & \textbf{87.8} & \textbf{88.6} & 168 & &  \textbf{96.1}  &  \textbf{93.7}  &  \textbf{85.9} & 84.8 & 221 & & 98.4 & \textbf{95.9} & 97.7 & \textbf{95.3} & 522 & &  86.3   & \textbf{66.0}     & \textbf{78.4}     & \textbf{74.5}     &     86\\ \midrule
Finch~\cite{finch}                                       & OC                        & 90.8  &  80.5     &   46.1    &    44.2   & \multirow{5}{*}{}&  & 82.9  &   75.3    &   49.6    &   41.0    & \multirow{5}{*}{} & & 92.2   &  89.9     &     85.2  &    85.6   & \multirow{5}{*}{} & &  81.6 &  58.6    &  \textbf{59.8}    &     56.8 & \multirow{5}{*}{}  \\
BCL~\cite{ball}                                         & OC                        & 94.0    & 85.0    &   -    &      - &  &  & 86.5  & 77.6  &  -     &  -     &  &   &    -   &    -   &   -    &      - &   &  &  -    &    -  &      -&     - &   \\
C1C~\cite{Kalogeiton20}                                         & OC                        & 95.3  & 84.5  &   54.9    &  57.3   &    & & 88.1  & 79.1  &    58.1   &  55.4     &    & & 94.3 & 93.2 & 79.1  & 85.5 &   & &  81.6 & 53.8 &     40.5 & 51.7     &    \\
\mnameMM--                                      & OC                        & \textbf{99.1}  & \textbf{97.4}  & \textbf{79.3}  & \textbf{83.0}  &   & & \textbf{95.6}  &  92.2  & \textbf{72.3}  & \textbf{73.8}  &    & & 96.3 & 92.7 & 89.0  & 88.8  & &    & 84.0 & 56.5 & 55.4 & 59.9 &    \\
\mnameMM (\textbf{ours})                                     & OC           &   \textbf{99.1}    &  \textbf{97.4}     &   \textbf{79.3}    & \textbf{83.0}  &  &   &  \textbf{95.6}       &  \textbf{93.1}       &    71.5   &    73.2   &  &   &  \textbf{97.1}     & \textbf{94.6}      &    \textbf{92.3}   & \textbf{92.6}      &  &   &    \textbf{85.1}  &     \textbf{63.9} & 59.6     &  \textbf{62.9}    &    \\ \bottomrule
% MM-HPC3                                     & OC      &       &       &       &       & "   &       &       &       &       & "   &       &       &       &       & "   &      &      &      &      & "  \\ \bottomrule
\end{tabular}
}%}
%}
%\vspace{-2mm}
\caption{\footnotesize{
\textbf{Face Clustering Results.} Comparisons to previous state of the art on four datasets, using only face-tracks. We experiment with unknown (AT), and known (OC) number of clusters. We report metrics averaged over each episode in each dataset, and the number of predicted clusters, summed over each episode of the dataset ($\#C_p$). 
MM-HPC-- uses only face, 
whereas MM-HPC uses the multi-modal bridges for body and voice. Where not reported in respective publications, additional numbers are computed using official implementations. Finch has no stopping criterion so results for AT are not reported.}}
\vspace{-2mm}
\label{tab:face_results}
\end{table*}



==> tables/person_clustering.tex <==
\begin{table*}[ht!]
\centering
\resizebox{\linewidth}{!}{
\footnotesize{
\begin{tabular}{llccc|cc|ccccccccccccccccccc}
\toprule
\# & Method & \multicolumn{3}{c|}{Modalities} & \multicolumn{2}{c|}{Bridging}   & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{TBBT}}  }       &\cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}}  &                                                             & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Buffy}} }        &          \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 165}}                  &                                & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Sherlock}}}  &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 50}}  &  & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Friends}}} & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 239}}\\ 
%%%%%%%%%%%%%%%%%%%%
& \multicolumn{1}{l}{} & face & body & voice  & face-body & face-voice  & WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & & 
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & & 
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & &
WCP                  & NMI                  & CP                 & CR \\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
i & \multirow{2}{*}{Baseline} &  & \checkmark & & &  &  66.2             &       54.9               &       11.4               & \multicolumn{1}{c}{33.0} &    &        52.0             &       48.8               &       40.6               & \multicolumn{1}{c}{24.6}  &  &         60.3             &          24.0            &        10.7              & \multicolumn{1}{c}{36.0}   &  &        62.8              &           56.0           &       49.8               & 56.4    \\ 
ii & &  \checkmark & \checkmark & & &  &     91.7          &       79.1               &       54.4              & \multicolumn{1}{c}{55.9}    &   &  74.5               &     62.7                                & \multicolumn{1}{c}{46.8}    &         44.7         &                   &      77.1               & \multicolumn{1}{c}{44.4}    &   33.2                 &          43.3          &                     &  88.0  &   82.4 & 74.5 & 78.9    \\ \hline
%%%%%%%%%%%%%%%%%%%%
iii & \multirow{3}{*}{\mnameMM}  &   \checkmark & \checkmark & & &   &    \textbf{97.0}              &         92.9             &         \textbf{77.6}             & \multicolumn{1}{c}{79.6}  &   &          \textbf{86.4}            &         76.3             &         69.5             & \multicolumn{1}{c}{69.9}  &   &           80.3           &         47.4             &         46.8             & \multicolumn{1}{c}{49.7}    & &              90.0        &             82.3         &             \textbf{88.4}         & 82.6    \\
%%%%%%%%%%%%%%%%%%%
iv &  & \checkmark & \checkmark &   &  \checkmark &  &     \textbf{97.0}            &          92.9            &      76.7                & \multicolumn{1}{c}{79.5}  &   &       85.9 &  76.1             &           69.0           &        \multicolumn{1}{c}{69.5}   &  &      79.4                &       50.9               &     58.6                 & \multicolumn{1}{c}{53.3}  &   &     89.5                 &      82.8               &        87.1           &    83.1    \\
 %%%%%%%%%%%%%%%%%%%%%%%%%% second row
v &  & \checkmark &\checkmark  & \checkmark &  & \checkmark &      96.8               &     \textbf{93.2}                 &     76.9                 & \multicolumn{1}{c}{79.1}    & &           86.0           &      76.6               &       69.8               & \multicolumn{1}{c}{70.6}   &  &     78.5                 &        50.3              &          57.4            & \multicolumn{1}{c}{\textbf{55.1}}    & &   \textbf{90.8}                   &     83.4                 &          87.0            & \textbf{85.4}  \\  \hline 
%%%%%%%%%%%%%%%%
vi & \cellcolor{mistyrose}{\mnameMM} &  \checkmark & \checkmark &  \checkmark & \checkmark & \checkmark &      96.8             &        \textbf{93.2   }           &        76.6              & \multicolumn{1}{c}{\textbf{79.6}}   &  &      86.0                &         \textbf{77.4}             &       \textbf{69.9}              & \multicolumn{1}{c}{\textbf{70.7}}  &   &      \textbf{ 80.5}               &       \textbf{53.7}               &        \textbf{ 59.9   }          & \multicolumn{1}{c}{53.6}  &   &            89.9        &        \textbf{83.5}             &      88.3              & 84.9     \\
\bottomrule
%%%%%%%%%%%%%%%%%%%%%%%% new one
%%%%%%%%%%%%%%%%%%%%%%%%
\# &Method & \multicolumn{3}{c|}{Modalities} & \multicolumn{2}{c|}{Bridging}   &  \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Hidden Figures}}}   & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 10}}  & & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{About Last Night}} } &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 24}}    & &  \multicolumn{4}{c}{{\textbf{}}} & &  \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Average}} } & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 618}}                                                                 \\ 
%%%%%%%%%%%%%%%%%%%%
& \multicolumn{1}{l}{} & face & body & voice  & face-body & face-voice  & WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR}  & & WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} &  &                   &                   &                  & \multicolumn{1}{c}{} &  &
WCP                  & NMI                  & CP                 & CR                  \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%
i &\multirow{2}{*}{Baseline} &  & \checkmark & & &  &                  33.7          &           10.5          &           17.6           & \multicolumn{1}{c}{31.7}    & &                27.3      &       17.9               &       19.9               & \multicolumn{1}{c}{19.3}   &  &                     &                    &                  &       \multicolumn{1}{c}{}   &      & 50.4 & 35.4 & 25.0 & 33.5      \\ 
ii & &  \checkmark & \checkmark & & &        &      69.5              &     51.8               &               29.7       & \multicolumn{1}{c}{46.4}    &                     &       73.1             &     \textbf{64.8}              & \multicolumn{1}{c}{55.7}    &              53.8     &                     &                 & \multicolumn{1}{c}{}    &                     &                     &                  &      79.0 & 64.2 & 49.1 & 53.8 \\ 
\hline
iii & \multirow{3}{*}{\mnameMM}   &   \checkmark & \checkmark & & &       &            71.9          &         61.8             &         56.9             & \multicolumn{1}{c}{48.4}  &   &    81.6                  &         60.1             &         60.7           &  \multicolumn{1}{c}{70.8}  &   &                      &                      &                 & \multicolumn{1}{c}{}  &   &      84.5 & 70.1 & 66.7 & 66.8                \\
%%%%%%%%%%%%%%%%%%%
iv & & \checkmark & \checkmark &   &  \checkmark &  &               \textbf{73.4 }               &       \textbf{ 63.8 }             &         \textbf{ 62.7   }         & \multicolumn{1}{c}{\textbf{50.8}}   &  &        82.2              &        61.8              &          70.7            & \multicolumn{1}{c}{78.8}  &   &                      &                      &      &        \multicolumn{1}{c}{}   &      &       84.6 & 71.4 & 70.8 & 69.2               \\
 %%%%%%%%%%%%%%%%%%%%%%%%%% second row
v & & \checkmark &\checkmark  & \checkmark &  & \checkmark &         71.8            &         62.1            &         55.0             & \multicolumn{1}{c}{47.2}   &  &      \textbf{82.6}               &        62.6              &            \textbf{88.2}          & \multicolumn{1}{c}{\textbf{80.0}}   &  &                      &                      &          &        \multicolumn{1}{c}{}  &   &          84.4 & 71.4 & 72.4 & 69.6            \\ \hline
%%%%%%%%%%%%%%%%
vi & \cellcolor{mistyrose}{\mnameMM} &  \checkmark & \checkmark &  \checkmark & \checkmark & \checkmark &         73.2             &        \textbf{63.8}           &           57.0           & \multicolumn{1}{c}{48.3}  &   &             \textbf{82.6}         &       62.6               &       \textbf{88.2}               & \multicolumn{1}{c}{\textbf{80.0}}  &   &                      &                      &         &          \multicolumn{1}{c}{}   & &          \cellcolor{mistyrose}{\textbf{84.8}} & \cellcolor{mistyrose}{\textbf{72.4}} & \cellcolor{mistyrose}{\textbf{73.3}} & \cellcolor{mistyrose}{\textbf{69.5}}            \\
 \bottomrule
\end{tabular}
}}
\vspace{-2mm}
\caption{\footnotesize{\textbf{Person Clustering Results.} Clustering results for the OC protocol on \datasetname. For TV-shows, each metric is averaged across all episodes. The Average is averaged across all datasets. $\#C_s$ is the sum number of ground truth clusters across each episode in the dataset. We report two strong baselines (i, ii, Section~\ref{sec:experiments}) and an ablation of multi-modal bridges from Stage 2. \textit{Modalities}: which modalities are used. \textit{Bridging}: which (if any) multi-modal bridges from Stage 2 are used.  }}
\vspace{-2mm}
\label{tab:person_results}
% Results on the proposed \datasetname. Method 1 is not using any of the multi-modal bridges in Stage 2. Method 2 is using the bridges. Baseline 1: We replace the primary modality in Stage 1 with the body modality, using the same MovieNet trained features. Method 3: We replace these features with powerful person Re-ID features. 
\end{table*}


==> tables/person_clustering2.tex <==
\begin{table*}[ht!]
\centering
\resizebox{\linewidth}{!}{
\footnotesize{
\begin{tabular}{llccc|cc|cccc ccccc ccccc ccccc ccccc ccccc ccccc}
\toprule
\# & Method & \multicolumn{3}{c|}{Modalities} & \multicolumn{2}{c|}{Bridging}   & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{TBBT}}  }       &\cellcolor{lavenderblue}{\textbf{$\#C_s$ = 130}}  &                                                             & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Buffy}} }        &          \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 165}}                  &                                & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Sherlock}}}  &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 50}}  &  & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Friends}}} & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 239}} 
& & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Hidden Figures}}}   & \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 10}}  & & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{About Last Night}} } &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 24}}    
& &  \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{Average}} } &  \cellcolor{lavenderblue}{\textbf{$\#C_s$ = 618}}
\\ 
%%%%%%%%%%%%%%%%%%%%
& \multicolumn{1}{l}{} & F & B & V  & F-B & F-V  & 
WCP   & NMI                  & CP                 & \multicolumn{1}{c}{CR} & & 
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & & 
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & &
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & &
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & &
WCP                  & NMI                  & CP                 & \multicolumn{1}{c}{CR} & &
WCP                  & NMI                  & CP                 & CR \\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
i & \multirow{2}{*}{Baseline} &  & \checkmark & & &  &  66.2             &       54.9               &       11.4               & \multicolumn{1}{c}{33.0} &    &        52.0             &       48.8               &       40.6               & \multicolumn{1}{c}{24.6}  &  &         60.3             &          24.0            &        10.7              & \multicolumn{1}{c}{36.0}   &  &        62.8              &           56.0           &       49.8               & 56.4  & &  33.7          &           10.5          &           17.6           & \multicolumn{1}{c}{31.7}    & &                27.3      &       17.9               &       19.9               & \multicolumn{1}{c}{19.3}    &      & 50.4 & 35.4 & 25.0 & 33.5   \\
%%%%%%%%%%%%%%%%%%%%%%%%%%% 
ii & &  \checkmark & \checkmark & & &  &     91.7          &       79.1               &       54.4              & \multicolumn{1}{c}{55.9}    &   &  74.5               &     62.7                                & \multicolumn{1}{c}{46.8}    &         44.7         &                   &      77.1               & \multicolumn{1}{c}{44.4}    &   33.2                 &          43.3          &                     &  88.0  &   82.4 & 74.5 & 78.9  & & 
69.5              &     51.8               &               29.7       & \multicolumn{1}{c}{46.4}    &                     &       73.1             &     \textbf{64.8}              & \multicolumn{1}{c}{55.7}    &              53.8            &                  &      79.0 & 64.2 & 49.1 & 53.8 
\\ 
%\hline
%%%%%%%%%%%%%%%%%%%%  
iii & \multirow{3}{*}{\mnameMM}  &   \checkmark & \checkmark & & &   &    \textbf{97.0}              &         92.9             &         \textbf{77.6}             & \multicolumn{1}{c}{79.6}  &   &          \textbf{86.4}            &         76.3             &         69.5             & \multicolumn{1}{c}{69.9}  &   &           80.3           &         47.4             &         46.8             & \multicolumn{1}{c}{49.7}    & &              90.0        &             82.3         &             \textbf{88.4}         & 82.6 & & 71.9          &         61.8             &         56.9             & \multicolumn{1}{c}{48.4}  &   &    81.6                  &         60.1             &         60.7           &  \multicolumn{1}{c}{70.8}  &   &      84.5 & 70.1 & 66.7 & 66.8       \\
%%%%%%%%%%%%%%%%%%%  
iv &  & \checkmark & \checkmark &   &  \checkmark &  &     \textbf{97.0}            &          92.9            &      76.7                & \multicolumn{1}{c}{79.5}  &   &       85.9 &  76.1             &           69.0           &        \multicolumn{1}{c}{69.5}   &  &      79.4                &       50.9               &     58.6                 & \multicolumn{1}{c}{53.3}  &   &     89.5                 &      82.8               &        87.1           &    83.1   &  & 
\textbf{73.4 }               &       \textbf{ 63.8 }             &         \textbf{ 62.7   }         & \multicolumn{1}{c}{\textbf{50.8}}   &  &        82.2              &        61.8              &          70.7            & \multicolumn{1}{c}{78.8}  &   &       84.6 & 71.4 & 70.8 & 69.2              
\\
 %%%%%%%%%%%%%%%%%%%%%%%%%% second row 
v &  & \checkmark &\checkmark  & \checkmark &  & \checkmark &      96.8               &     \textbf{93.2}                 &     76.9                 & \multicolumn{1}{c}{79.1}    & &           86.0           &      76.6               &       69.8               & \multicolumn{1}{c}{70.6}   &  &     78.5                 &        50.3              &          57.4            & \multicolumn{1}{c}{\textbf{55.1}}    & &   \textbf{90.8}                   &     83.4                 &          87.0            & \textbf{85.4}  & & 
71.8            &         62.1            &         55.0             & \multicolumn{1}{c}{47.2}   &  &      \textbf{82.6}               &        62.6              &            \textbf{88.2}          & \multicolumn{1}{c}{\textbf{80.0}}      & &          84.4 & 71.4 & 72.4 & 69.6   
\\  \hline 
%%%%%%%%%%%%%%%%
vi & \cellcolor{mistyrose}{\textbf{\mnameMM}} &  \checkmark & \checkmark &  \checkmark & \checkmark & \checkmark &      96.8             &        \textbf{93.2   }           &        76.6              & \multicolumn{1}{c}{\textbf{79.6}}   &  &      86.0                &         \textbf{77.4}             &       \textbf{69.9}              & \multicolumn{1}{c}{\textbf{70.7}}  &   &      \textbf{ 80.5}               &       \textbf{53.7}               &        \textbf{ 59.9   }          & \multicolumn{1}{c}{53.6}  &   &            89.9        &        \textbf{83.5}             &      88.3              & 84.9    & & 
 73.2             &        \textbf{63.8}           &           57.0           & \multicolumn{1}{c}{48.3}  &   &             \textbf{82.6}         &       62.6               &       \textbf{88.2}               & \multicolumn{1}{c}{\textbf{80.0}}  &   &          \cellcolor{mistyrose}{\textbf{84.8}} & \cellcolor{mistyrose}{\textbf{72.4}} & \cellcolor{mistyrose}{\textbf{73.3}} & \cellcolor{mistyrose}{\textbf{69.5}}           
 \\
\bottomrule
\end{tabular}
}}
%\vspace{-2mm}
\caption{\footnotesize{\textbf{Person Clustering Results.} Clustering results for the OC protocol on \datasetname. For TV-shows, each metric is averaged across all episodes. The Average is averaged across all datasets. $\#C_s$ is the sum number of ground truth clusters across each episode in the dataset. We report two strong baselines (i, ii, Section~\ref{sec:experiments}) and an ablation of multi-modal bridges from Stage 2. \textit{Modalities}: which modalities are used. \textit{Bridging}: which (if any) multi-modal bridges from Stage 2 are used.  }}
\vspace{-2mm}
\label{tab:person_results}
% Results on the proposed \datasetname. Method 1 is not using any of the multi-modal bridges in Stage 2. Method 2 is using the bridges. Baseline 1: We replace the primary modality in Stage 1 with the body modality, using the same MovieNet trained features. Method 3: We replace these features with powerful person Re-ID features. 
\end{table*}

